Uniqueness of Lagrangians in $T^*RP2$

We present a new and simpler proof of the fact that any Lagrangian $\mathbb{R}P^2$ in $T^*\mathbb{R}P^2$ is Hamiltonian isotopic to the zero section. Our proof mirrors the one given by Li and Wu for the Hamiltonian uniqueness of Lagrangians in $T^*S^2$, using surgery to turn Lagrangian spheres into symplectic ones. The main novel contribution is a detailed proof of the folklore fact that the complement of a symplectic quadric in $\mathbb{C}P^2$ can be identified with the unit cotangent disc bundle of $\mathbb{R}P^2$.

==> Recolections_on_the_Rational_Blow_up.tex <==
The rational blow-up and blow-down are surgeries performed in $4$-manifolds, originally introduced by Fintushel-Stern in \cite{FS}. Roughly speaking, the idea is to look at certain configurations of spheres $C=\cup S_i$ and to consider different fillings of the 3-manifold $Y$ that appears as the boundary of a tubular neighborhood of $C$. For instance, different fillings may come from viewing $Y$ as the link of a smoothable surface singularity. Considering $C$ as the exceptional divisor of the resolution, another filling is obtained by the Milnor fiber (or smoothing) of the singularity. In fact, the usual Blow-up can be seen as a trivial instance of the above idea, where the isolated singularity is already smooth.\par

Rationally blowing-up/down can also be done in a symplectic manner under suitable conditions, as shown first by Symington \cite{Sym}. The reader is also referred to \cite{evans_2023} for a more modern exposition. For us, the relevant cases are when $C$ consists of a single $(+2)$ or $(+4)$ symplectic sphere, and blowing down $C$ will replace it with a Lagrangian $S^2$ or $\mathbb{R}P^2$ respectively. Conversely, blowing up such a Lagrangian $L$ will replace it with the corresponding symplectic sphere $C$. The power of this technique comes from the following simple observation with many surprising applications.


\begin{proposition}\emph{(\cite{LW},\cite{BLW})}\label{rblowup}
Let $L$ be either a Lagrangian $S^2$ or $\mathbb{R}P^2$ in a symplectic $4$-manifold $(M,\omega)$. Rationally blowing up $L$ produces a new symplectic manifold $(\widetilde{M},\widetilde{\omega})$ where $L$ has been replaced by $S$, a symplectic $(-2)$ or $(-4)$-sphere respectively. In addition, if $M$ is rational, then so is $\widetilde{M}$.
\end{proposition}

\begin{remark}
Since blowing-up along $L$ alters $M$ only in a small neighborhood of $L$, it is clear that $(M-\nu L,\omega)$ is symplectomorphic to $(\widetilde{M}-\nu S,\widetilde{\omega})$, where $\nu L$ and $\nu S$ are small enough standard Weinstein neighborhoods of the corresponding submanifolds.
\end{remark}

One instance where the above remark becomes useful is that symplectic behavior \textit{relative} to $L$ is the same as relative to $S$. For example, in section 6.4.1 in \cite{LW}, the following is shown:

\begin{lemma}\label{sphereuniq}
Any two symplectic $(+4)$-spheres in $(\mathbb{C}P^2,\omega_{FS})$ disjoint from the standard $\mathbb{R}P^2$ are Hamiltonian isotopic via an isotopy that fixes the Lagrangian $\mathbb{R}P^2$.
\end{lemma}

Another and arguably more important, application of Proposition \ref{rblowup} is the proof of Hamiltonian uniqueness of spheres or projective spaces in certain symplectic rational manifolds.

\begin{Theorem}\emph{(\cite{H}, Section 6 in \cite{LW}, Theorem 1.3 in \cite{BLW})}\label{laguniqcp2}
Any two Lagrangian $\mathbb{R}P^2$s in $(\mathbb{C}P^2,\omega_{FS})$ are Hamiltonian isotopic.
\end{Theorem}






==> S2xS2.tex <==
\par 
In his famous paper \cite{Gr85}, Gromov computed for the first time the symplectomorphism group of a symplectic $4$-manifold, namely $(S^2\times S^2,\sigma\times \sigma)$. He showed that this group has the homotopy type of $(SO(3)\times SO(3))\rtimes \mathbb{Z}/2$. This is a central result because the unit polydisc $D^2\times D^2\subset \mathbb{C}^2$ naturally compactifies to $S^2\times S^2$. He also argued that when the product factors are of uneven area, the topology of the symplectomorphism group changes dramatically. For example, it becomes connected and not simply connected. These observations where further developed by many people, with M. Abreu and D. McDuff bringing some of the most central results. Among other, they computed the topology of the symplectomorphism groups of symplectically ruled surfaces and also showed that any two cohomologous forms on these surfaces are actually diffeomorphic to each other.\par
The first result we need was shown by Abreu in \cite{Ab}. It states that symplectic spheres in the homology class of the antidiagonal of $S^2\times S^2$ $\bar\Delta$ are unique up to isotopy. Thus, in particular, we have:
\begin{Theorem}\label{tracsy}
Let $S^2\times S^2$ be equipped with the unevenly weighted product symplectic form $(1+\lambda)\omega\oplus \omega, \lambda>0$. Then, any two embedded symplectic spheres in the homology class of the antidiagonal may be mapped to each other by a symplectomorphism. 
\end{Theorem}
\begin{proof}
See Lemma $3.5$ in \cite{Ab}. $\square$
\end{proof}
The second theorem we need, proved by Hind and Irvii in \cite{HI} can be seen as a generalization of the above theorem, as it establishes uniqueness up to symplectic isotopy for symplectic spheres in the homology class not only of $\bar\Delta$ but also of $\Delta$, when $S^2\times S^2$ is equipped with a symplectic form that turns it in a symplectically ruled surface. 
\begin{Theorem}\label{hindtheorem}
Let $S_-,S_+$ be disjoint, embedded symplectic spheres in the homology class of $\bar{\Delta}$ and $\Delta$ respectively. Then, any third embedded symplectic sphere in the homology class of $S_\pm$ and disjoint from $S_\mp$ is symplectically isotopic to $S_\pm$, through an isotopy that stays away from $S_\mp$.
\end{Theorem}
\begin{proof}
See Theorem $8.1$ in \cite{HI}.$\square$
\end{proof}

Even though the second theorem might seem stronger at first sight (since it establishes uniqueness for both homology classes) to use it we have to establish that the symplectic sphere we want to isotope must be disjoint from another symplectic sphere in the \say{opposite} homology class, whose existence also has to be ensured. No such requirement is needed for Theorem $\ref{tracsy}$ and this is precisely why both of them are useful to us.








% In this section, we collect certain useful facts concerning symplectic spheres in $S^2\times S^2$. 

% The relevant uniqueness theorem for symplectic spheres in $S^2\times S^2$ is due to Hind and Irvii (\cite{HI}). Their theorem states that in $S^2\times S^2$, when equipped with a symplectic form that turns it into a symplectically ruled surface, symplectic spheres in the class of $\bar{\Delta}$ or $\Delta$ are unique.
% \begin{Theorem}\label{hindtheorem}
% Let $S_-,S_+$ be disjoint, embedded symplectic spheres belonging in the homology class of $\bar{\Delta}$ and $\Delta$ respectively. Then, any third embedded symplectic sphere in the homology class of $S_\pm$ and disjoint from $S_\mp$ is symplectically isotopic to $S_\pm$, through an isotopy that stays away from $S_\mp$.
% \end{Theorem}
% \begin{proof}
% See Theorem $8.1$ in \cite{HI}.
% \end{proof}
% Even though the above theorem is very useful, it has a shortcoming: To use it, one needs to establish the existence of the two \say{opposite} symplectic spheres $S_-$ and $S_+$. In fact, we will need to establish uniqueness of symplectic spheres in the homology class of $\bar\Delta$, without finding an $S_+$. This was shown by Abreu in \cite{Ab}. In particular, we have
% \begin{proposition}\label{tracsy}
% Let $S^2\times S^2$ be equipped with the unevenly weighted product symplectic form $(1+\lambda)\omega\oplus \omega, \lambda>0$. Then, any two embedded symplectic spheres in the homology class of the antidiagonal may be mapped to each other by a symplectomorphism. 
% \end{proposition}
% \begin{proof}
% See Lemma $3.5$ in \cite{Ab}. $\square$
% \end{proof}







% The reason this is relevant is that, roughly, the complement of a Lagrangian $\mathbb{R}P^2$ in $\mathbb{C}P^2$ is symplectomorphic to the complement of a symplectic $(-2)$ sphere in $S^2\times S^2$. Therefore the uniqueness of Lagrangians in $\mathbb{C}P^2$ will be based on establishing uniqueness for symplectic spheres in the homology class of the anti-diagonal.\par
% Let us briefly explain how this works. By the Weinstein Lagrangian Neighborhood Theorem, a neighborhood of a Lagrangian $\mathbb{R}P^2$ is symplectomorphic to a radius $r$ cotangent disc bundle of $\mathbb{R}P^2$, denoted by $U^*_r\mathbb{R}P^2$. Since all geodesics of $\mathbb{R}P^2$ are periodic with the same period, the normalized (co)-geodesic flow induces a Hamiltonian $S^1$-action on the cotangent bundle. Now, the boundary of the cotangent discs may be symplectically cut, or in other words, reduced, to a symplectic sphere. Thus, by using symplectic cut, we are able to replace a Lagrangian $\mathbb{R}P^2$ with a symplectic $(+2)$-sphere. In the case that the Lagrangian $\mathbb{R}P^2$ lies in $\mathbb{C}P^2$ this process transforms $\mathbb{C}P^2$ to $S^2\times S^2$. This is the content of 
% \begin{proposition}
% \label{cohodiffeo}
% Let $(\widetilde{M}_1,\omega_1)$ and $(\widetilde{M}_2,\omega_2)$ be two symplectic manifolds that result from surgery on Lagrangians $L_1,L_2$ disjoint from a symplectic sphere $S$ of degree $2$. Then $(\widetilde{M}_1,\omega_1)$ is symplectomorphic to $(\widetilde{M}_2,\omega_2)$. In particular, both are symplectomorphic to $(S^2\times S^2, (1+\lambda)\sigma\oplus\sigma)$ with $\lambda>0$.
% \end{proposition}
% \begin{proof}
% The manifolds $(\widetilde{M}_i,\omega_i)$ carry no $(-1)$-symplectic sphere and therefore, by a theorem of McDuff (see Theorem $9.4.1$ in \cite{McDS}), are both symplectomorphic to a symplectically ruled manifold. Since both contain the same symplectic sphere of degree $2$ (coming from $S$) and since the surgery can be arranged to be made on the same radius $r$ of the normal bundles of the $L_i$, wee see that the $\omega_i$ represent the same cohomology class. Another theorem of McDuff (for example, Theorem $2.3$ in \cite{LaMcD}) states that any two cohomologous forms on a symplectically ruled surface are diffeomorphic. Thus, the $(\widetilde{M}_i,\omega_i)$ are symplectomorphic.\par
% The last statement follows by the classification of symplectic forms on $S^2\times S^2$ as done in \cite{Ab}. $\square$
% \end{proof}

==> compactif.tex <==
To make Proposition $\ref{lagmap}$ a statement about $T^*\mathbb{R}P^2$ we will argue as follows: First, we prove a general compactification procedure that works in all dimensions. The problem with this compactification is that even though it identifies the radius $r$ cotangent disc bundle of the projective space (denoted by $U^*_r\mathbb{R}P^n$) with a complement of the Fermat quadric $Q^{n-1}=[\sum z_i^2=0]$ in $\mathbb{C}P^n$, in order to make this work $\mathbb{C}P^n$ is endowed with a form that is \textbf{not} the Fubini Study form. Nevertheless, we will show that, in dimension $4$, this form is indeed diffeomorphic to the Fubini Study form, appropriately scaled. In its most general form, our compactification theorem identifies any Lagrangian $\mathbb{R}P^2\subset \mathbb{C}P^2$ with the zero section of the cotangent bundle and the rest of $U_r^*\mathbb{R}P^2$ with the complement of any symplectic sphere of degree $2$ disjoint from the Lagrangian. \par
Let us first establish some conventions. We will identify $T^*S^n$ with the subset of $(\mathbb{R}^{n+1}\oplus\mathbb{R}^{n+1},\omega_{std})$ defined as
\[\{(p,q)\big||p|=1,\langle p,q\rangle=0\}\subset \mathbb{R}^{n+1}\oplus\mathbb{R}^{n+1}.\]
As we mentioned above, the compactification will involve the  $2n$-dimensional quadric $Q^n\subset \mathbb{C}P^{n+1}$. In $\mathbb{C}P^n$ we will denote by $H_i$ the hyperplane defined by the vanishing of the $i$-th coordinate. Notice that the hyperplane $H_i\subset \mathbb{C}P^{n+1}$ intersects $Q^n$ in a quadric which may (and will) be identified with $Q^{n-1}$.\par
The results of this sections were inspired by Audin's paper \cite{AuLag}, section $4$. We adopt a different method of proof to show the compactification, which might be less natural but we feel is more precise and straightforward and, at the same time, makes explicit how the symplectic form on the compactification changes as we alter the radius of the disc bundle that we care to compactify.


\subsection{The general construction}
The idea for the general compactification is simple. First, recall that the ball of $\mathbb{C}^{n}$ may be symplectically identified with the complement of a hyperplane $H_{n}$ in $\mathbb{C}P^n$. We will place $U_1^*S^n$ inside a ball of $\mathbb{C}^{n+1}$ such that the boundary of $U_1^*S^n$ will be a subset of the boundary of the ball. Thus, placing the ball inside $\mathbb{C}P^n$ will identify $U^*S^n$ with the quadric $Q^n$ and the boundary of $U_1^*S^n$ will be mapped to $Q^{n-1}\subset Q^{n}$, thus realizing the aforementioned diffeomorphism in a symplectic manner.\par
First, let us explain how how to symplectically embedd a ball in $\mathbb{C}P^n$.
\begin{lemma}\label{projemb}
The open ball of radius $r$, $(B(r),\omega_{std})\subset \mathbb{C}^{n+1}$, is symplectomorphic to $\mathbb{C}P^{n+1}-H_{n+1}$ with the form $r^2\omega_{FS}$.
\end{lemma}
\begin{proof}
Consider the map $\phi:B^{2n+2}(r)\rightarrow \mathbb{C}P^{n+1}\backslash H_{n+1}$ given by 
\[\phi(z_0,\dots z_n)=[z_0:\dots:z_n:i\sqrt{r^2-\sum |z_i|^2}].\]
This map lifts to a map $\bar{\phi}$ to $S(r)\subset \mathbb{C}^{n+2}$. Denoting by $i_r:S(r)\hookrightarrow \mathbb{C}^{n+1}$ the inclusion of the sphere of radius $r$, $S(r)$, to $\mathbb{C}^{n+2}$ and with $\pi_r$ the projection of $S(r)$ to $\mathbb{C}P^{n+1}$ we have that \[r^2\pi_r^*\omega_{FS}=i_r^*\omega_{std}.\]
Therefore we readily compute
\begin{align*}
    \phi^*\omega_{FS}&=\bar{\phi}^*\pi_r^*\omega_{FS}\\
                     &=\frac{1}{r^2}\bar{\phi}^*i_r^*\omega_{std}\\
                     &=\frac{1}{r^2}\omega_{std}.
\end{align*}
To see why the last equality holds, just put coordinates $z_k=x_k+iy_k$ and notice that $x_{n+1}\circ\big(i_r\circ\bar\phi\big)=0$.$\square$
\end{proof}
Now, notice that $U^*_1S^n\subset B(\sqrt{2})\subset \mathbb{C}^{n+1}$. Therefore using the above map we can prove
\begin{lemma}\label{sphereembedding}
$(U^*_1S^n,\omega_{std})$ is symplectomorphic to $Q^n-Q^{n-1}$ with the restriction of the form $2\omega_{FS}$.
\end{lemma}
\begin{proof}
All we have to show is that the map $\phi(z_1,\dots,z_n)=[z_1:\dots:z_n:i\sqrt{2-\sum|z_i|^2}]$
maps $U^*S^n$ to $Q^n-Q^{n-1}$. For $[z_0:\dots,z_{n-1},z_{n}]\in \mathbb{C}P^{n+1}\backslash H_{n+1}$ we then have
\begin{align*}
   z_1^2+\dots+z_n^2+z_{n+1}^2&=z_1^2+\dots+z_n^2-2+\sum|z_k|^2\\
   &=\sum_1^n (x_k^2-y_k^2)+2i\sum_1^n  x_ky_k-2+\sum_1^n(x_k^2+y_k^2)\\
                                   &=2(\sum_1^nx_k^2-1)+2i\sum_1^nx_ky_k
\end{align*}
Therefore, elements of $Q^n-Q^{n-1}$ are the $\phi$-images of the elements $(x,y)$ of $B(\sqrt{2})$ that satisfy $|x|=1$ and $\langle x,y\rangle=0$ which is exactly $U^*TS^n$. $\square$
\end{proof}
We have proved that the \textit{interior} of the cotangent disc bundle is symplectomorphic to the complement of $Q^{n-1}$ in $Q^n$. Now, we would like to show that symplectically cutting the boundary (which in our language means \say{compactifying}) actually gives us $Q^n$. Therefore, we have 
\begin{proposition}\label{unitcut}
The symplectic cut on $H^{-1}(1)$ with the Hamiltonian $H:T^*S^n\rightarrow \mathbb{R}$, given by $H(u,v)=|v|$, is symplectomorphic to  $(Q^n,2\omega_{FS})$. 
\end{proposition}
\begin{proof}
Using the map $\phi$ of Lemma $\ref{sphereembedding}$ we see that the open unit cotangent bundle is symplectomorphic to $Q^n- Q^{n-1}$ inside $\mathbb{C}P^{n+1}$ with the form $2\omega_{FS}$.\par
Now, notice that the unit co-sphere bundle $S^*S^n$ is mapped to $Q^{n-1}\subset Q^n$. Indeed, the map $\phi$ extended to $S^*S^n$ gives the map 
\[(z_1,\dots,z_n)\rightarrow [z_1:\dots z_n:0].\]
The condition that the projective coordinates satisfy $\sum z_i^2=0$ is equivalent that the affine coordinates $z_k=x_k+iy_k$ satisfy $|x|^2=|y|^2$ and $\langle x,y \rangle=0$. Therefore $S^*S^n$ is mapped to $Q^{n-1}\subset \mathbb{C}P^{n+1}$.\par
So far we have constructed a map from the (closed) unit disc bundle to $Q^n$. To conclude that the symplectic cut is actually symplectomorphic to $Q^n$, we have to show that after the cut the reduced unit circle bundle is symplectomorphic to $Q^{n-1}$. This follows because the Hamiltonian action induced by $H$ on $S^*(S^n)\subset \mathbb{R}^{n+1}\oplus\mathbb{R}^{n+1}$ agrees with the Hamiltonian action by scalar multiplication on $S(\sqrt{2})$. Indeed, the trajectory of a point $(p,q)\in S^*S^n$ under the the action of $H$ is
\[\sigma_t(p,q)=(\cos(t)u+\sin(t)v,\cos(t)v-\sin(t)u)=e^{-it}\cdot(p,q).\]
$\square$
\end{proof}



So far we have only concerned ourselves with $T^*S^n$. We would like to use the compactification of $T^*S^n$ and the fact that $T^*S^n$ double covers $T^*\mathbb{R}P^n$ to deduce a compactification for $T^*\mathbb{R}P^n$. This is the content of
\begin{corollary}\label{branchedcovering}
Symplectically cutting on the double cover $U^*S^n\xrightarrow{p} U^*\mathbb{R}P^n$ we get a branched covering $Q^n\xrightarrow{\pi} \mathbb{C}P^n$.
\end{corollary}
\begin{proof}
First, let us examine the branched covering. We can define the map $\pi: \mathbb{C}P^{n+1}-[0:\dots:0,1]\rightarrow \mathbb{C}P^n$ simply by \[[z_0:\dots:z_n:z_{n+1}]\xrightarrow{\pi} [z_0:\dots:z_n].\]
When restricted to $Q^n$ this map gives a double cover $Q^n\rightarrow \mathbb{C}P^n$, branched along $Q^{n-1}\subset\mathbb{C}P^n$. The deck transformation of the cover is given simply by \[\delta:[z_0:\dots:z_{n+1}]\rightarrow [z_0:\dots:-z_{n+1}].\]
The inclusion $U^*S^n\xhookrightarrow{i} Q^n\backslash Q^{n-1}$ commutes with $\delta$ and with the antipodal action, i.e. $\delta\circ i (p,q)=i(-p,-q)$, therefore we can push down the symplectic form on $Q^n-Q^{n-1}$ to $\mathbb{C}P^{n}-Q^{n-1}$. As before, the inclusion extends to a map from the symplectically cut cotangent bundle to $\mathbb{C}P^n$. $\square$
\end{proof}
\begin{remark}
In the above corollary we showed that the symplectic covering $U^*_rS^n\rightarrow U^*_r\mathbb{R}P^n$ extends, via symplectic cut, to a symplectic branched covering $Q^n\rightarrow\mathbb{C}P^n$. Yet, as we have remarked before, the form $\omega_1$ (the subscript denoting the radius of the discs) we endow $\mathbb{C}P^n$ is \textbf{NOT} a multiple of the Fubini-Study form. This happens because the map $\pi$ above is a submersion and does not pullback the $\omega_{FS}$ of $\mathbb{C}P^n$ on the $\omega_{FS}$ of $\mathbb{C}P^{n+1}$. We will discuss this situation below in more detail.
\end{remark}

\subsection{Dimension $4$}
Let us not forget that we are actually interested to understand the geometry of the symplectic cut on dimension $4$. 
\begin{proposition}
$(Q^2,2\omega_{FS})$ is symplectomorphic to $(\mathbb{C}P^1\times\mathbb{C}P^1,2\omega_{FS}\oplus2\omega_{FS})$. 
\end{proposition}
\begin{proof}
Consider the map $\phi:\mathbb{C}P^1\times \mathbb{C}P^1\rightarrow \mathbb{C}P^3$ given by 
\[([x:y],[a:b])\xrightarrow{\phi} [xa+yb:i(xa-yb):i(xb+ya):xb-ya].\]
This is a symplectomorphism because it is the composition of the Segre embedding
\[([x:y],[a:b])\rightarrow [xa:xb:ya:yb]\]
with the projective map given by the unitary (up to scaling) matrix
\[
\begin{bmatrix}
1 & 0 & 0 & 1\\
i & 0 & 0 & -i\\
0 & i & i & 0\\
0 & i & -i & 0
\end{bmatrix}
.\]
Since the matrix is unitary, it imposes a symplectomorphism and it is well known that the Segre embedding pulls back the Fubini-Study form of $\mathbb{C}P^3$ to the product of the Fubini-Study forms on $\mathbb{C}P^1\times \mathbb{C}P^1$. $\square$
\end{proof}
\begin{remark}
Let $\iota$ by the swapping of factors. The map $\phi$ respects the involutions, namely, $\phi\circ\delta=\iota\circ \phi$. Straightforward calculations show that the map $\pi\circ\phi:\mathbb{C}P^1\times \mathbb{C}P^1\rightarrow \mathbb{C}P^2$ ($\pi$ being the branched covering we defined above)  sends symplectomorphically the diagonal $\Delta\subset \mathbb{C}P^1\times \mathbb{C}P^1$ to the quadric $Q^{1}\subset \mathbb{C}P^2$ and the antidiagonal covers $\bar{\Delta}$ the real projective space $\mathbb{R}P^2\subset\mathbb{C}P^2$. 
\end{remark}
An important matter is still open, and it is that the form $\omega_1$ we get on $\mathbb{C}P^2$ is not the Fubini-Study form. This will be resolved using  
\begin{proposition}
The form $\omega_1$ is symplectomorphic to $2\omega_{FS}$.
\end{proposition}
\begin{proof}
It is immediate that $\omega_1$ and $2\omega_{FS}$ are cohomologous thus diffeomorphic by a celebrated theorem of Taubes, which relies on the use of Seiberg-Witten invariants.\par
Alternatively, notice that our $(\mathbb{C}P^1,\omega_1)$ contains a symplectic sphere with positive self intersection, namely the quadric $Q^1$. Thus, one can use the much more elementary theorem of McDuff (Theorem 9.4.1 in \cite{McDS}) to deduce that the two forms are diffeomorphic. $\square$ 
\end{proof}
\begin{remark}
We think that it is very likely that the above situation holds in every dimension, i.e. $\omega_1$ is always symplectomorphic to $2\omega_{FS}$. Yet we were not able to prove this.
\end{remark}
\subsection{Compactifying with radius $r$}
For our purposes, we want to extend the above discussion in the disc bundle with arbitrary radius. We denote this by $U^*_r(S^n(1))$, or briefly, $U^*_r$. The proof of Proposition $\ref{unitcut}$ does not immediately generalize to our case. The reason is that, even though $S^*_r$ (namely the radius $r$ (co)-sphere bundle over $S^n(1)$) is a subset of $S^{2n-1}(\sqrt{1+r^2})\subset \mathbb{R}^{n+1}\times \mathbb{R}^{n+1}$, the action of the Hamiltonian $H(p,q)=|q|$ does not agree with the usual action by scalars on $S^{2n+1}$. Indeed, the trajectory of a point $(p,q)\in S^{2n+1}(\sqrt{1-r^2})$ under the action of $H$ is
\[\sigma_t(p,q)=(\cos(t)p+\frac{1}{r}\sin(t)q,\cos(t)q-r\sin(t)p)\]
while under the scalar action is
\[e^{-it}\cdot(p,q)=(\cos(t)u+\sin(t)v,\cos(t)v-\sin(t)u).\]
Notice that the agreement of this actions was crucial to prove Proposition $\ref{unitcut}$. The problem is that the discs have different radius than the base sphere.\par
Yet, we can do the following trick: The radius $r$ disc bundle over the unit sphere is symplectomorphic with the radius $\sqrt{r}$ disc bundle over $S^{n}(\sqrt{r})$ or, briefly, $S(\sqrt{r})$. The corresponding Hamiltonian that produces an $S^1$ action on $T^*S(k)$ is $H_k(p,q)=k|q|$. Therefore symplectic cut on the radius $r$ disc bundle over $S(1)$ is symplectomorphic to the the symplectic cut on the radius $\sqrt{r}$ disc bundle over $S(\sqrt{r})$. Notice that this \say{evened} disc bundle sits inside $B(\sqrt{2r})$, Now, all the above discussion transfers to our case and we have
\begin{proposition}$\label{almostcompactif}$
Symplectic cut along $(U^*_r(S^n(1)),\omega_{std})$ is symplectomorphic to $(Q^n,2r\omega_{FS})$. In addition, symplectic cut along $(U^*_r\mathbb{R}P^n,\omega_{std})$ gives rise to the (symplectic) branched cover $(Q^n,2r\omega_{FS})\rightarrow (\mathbb{C}P^n,\omega_r)$. 
\end{proposition}
\begin{remark}
Examining the branched cover $(Q^n,2r\omega_{FS})\rightarrow(\mathbb{C}P^n,\omega_r)$, one immediately sees that the map sends symplectomorphicaly the $Q^{n-1}$ (sitting inside $Q^n$) to $Q^{n-1}$ (sitting inside $\mathbb{C}P^n$). Thus, we have that 
\[\omega_{r}\big|_{Q^{n-1}}=2r\omega_{FS}\big|_{Q^{n-1}}\]
which implies that the forms $\omega_{r}$ and $2r\omega_{FS}$ are cohomologous. On first sight, this result might seem odd; Since the discs are scaled, one would expect that the form are scaled \textit{quadratically}. After all, the scaling map $\psi_r:(x,y)\rightarrow r(x,y)$ does exactly this: $\psi_r^*\omega_{std}=r^2\omega_{std}$. However, in our case, the discs get dilated \textit{only in the cotangent direction}, therefore it is logical that the form is also linearly dilated.
\end{remark}
The same discussion applies for dimension $4$, where we have
\begin{corollary}\label{rdiscbundle}
Symplectic cut along the radius $r$ discs of $U_r^*S^2\rightarrow U^*_r\mathbb{R}P^2$ gives the (symplectic) branched covering $(\mathbb{C}P^1\times\mathbb{C}P^1,2r\omega_{FS})\rightarrow (\mathbb{C}P^2,\omega_r)$. The form $\omega_r$ is symplectomorphic to $2r\omega_{FS}$.
\end{corollary}

\subsection{A general compactification statement}
Corollary $\ref{rdiscbundle}$ is not of much use by itself, since we do not know how the symplectomorphism that maps $\omega_r$ to $2r\omega_{FS}$ behaves. Yet, due to Corollary $\ref{sympair}$, this is not a real problem, since we can correct this symplectomorphism even further.
\begin{Theorem}\label{compacttheorem}
Let $L$ be a Lagrangian $\mathbb{R}P^2$ in  $\mathbb{C}P^2$ and $S$ a degree $2$ symplectic sphere such that $L\cap S=\emptyset$. Then $(U_r^*\mathbb{R}P^2,\omega_{std})$ is symplectomorphic to $(\mathbb{C}P^2-S,2r\omega_{FS})$ where $S$ is any degree $2$ symplectic sphere in $\mathbb{C}P^2$. The symplectomorphism may be chosen to map the zero section to $L$. In particular, $S$ can be taken to be $Q^1$ and $L$ to be the standard real projective plane.
\end{Theorem}
\begin{proof}
With all the machinery we have developed so far, the proof becomes trivial. Proposition $\ref{almostcompactif}$ shows that the radius $r$ cotangent disc bundle can be compactified to $\mathbb{C}P^2$ such that the zero section $0_s$ is mapped to the standard real projective plane and the boundary of the disc bundle is mapped to $Q^1$. Denote by $\psi$ a symplectomorphism such that $\psi^*(2r\omega_{FS})=\omega_r$, which exists by Corollary $\ref{rdiscbundle}$. Since $Q^1$ and the standard $\mathbb{R}P^2$ are disjoint, so are $S'=\psi(Q^1)$ and $L'=\psi(\mathbb{R}P^2)$. Therefore, using Corollary $\ref{sympair}$, $\psi$ can be further corrected to map the pair $(S',L')$ to any other disjoint pair $(S'',L'')$. In particular $(S'',L'')$ can be taken to be the standard pair $Q^1$ and $\mathbb{R}P^2$. $\square$.
\end{proof}

==> cp2.tex <==
\subsection{Surgery via Symplectic Cut}
Now, we will transform the above facts about the symplectic topology of $S^2\times S^2$ in facts about surfaces of $\mathbb{C}P^2$. Our main tool for this will be a kind of symplectic surgery called \textit{symplectic cut}.\par




Let us recall what symplectic cut is and explain how we will use it. Suppose we have a symplectic manifold $(M,\omega)$ and a Hamiltonian action induced by $H:M\rightarrow \mathbb{R}$ (we will only care about $S^1$-actions). Then, for any regular value $s$ of $H$, we consider the decomposition of $M$ in the sub/super-level sets $M_{\leq s}$ and $M_{\geq s}$. One may perform symplectic reduction at the level set of $s$ to get a reduced manifold $\widetilde{M}=H^{-1}(s)/\sim$. The key point is that one can actually perform symplectic cut on the whole sub/super level sets in such a way that the strict sub/super level sets stay intact but the level set gets reduced. This is achieved by cleverly performing symplectic reduction on $M\times \mathbb{C}$. Thus, one gets a new symplectic manifold $\widetilde{M}_{\leq,\geq s}$ having $\widetilde{M}$ as a symplectic hypersurface, such that we have a symplectic map of pairs 
\[(M_{\leq,\geq s},H^{-1}(s))\xrightarrow{\psi} (\widetilde{M}_{\leq,\geq s},\widetilde M)\]
where $\psi$, when restricted to $H^{-1}(s)$ is the symplectic reduction and when restricted to $M_{\leq,\geq s}$ is the identity. It is easy to see that the normal bundle of $\widetilde{M}$ inherits opposite orientation when seen as a subset of either $\widetilde{M}_{\leq s}$ or $\widetilde{M}_{\geq s}$. Thus, by performing symplectic sum \textit{\'a la Gompf} (\cite{Go}) along the different $\widetilde{M}$ we can recover the original symplectic manifold $M$. Symplectic cut and symplectic sum are, in this way, opposite operations. Symplectic cut was first defined by Lerman in \cite{Ler} and we refer the reader to this paper for more details.\par
We will use symplectic cut to turn a Lagrangian $\mathbb{R}P^2$ in a symplectic sphere in $S^2\times S^2$. Let us briefly explain how this works. By the Weinstein Lagrangian Neighborhood Theorem, a neighborhood of a Lagrangian $\mathbb{R}P^2$ is symplectomorphic to a radius $r$ cotangent disc bundle of $\mathbb{R}P^2$, denoted by $U^*_r\mathbb{R}P^2$. Since all geodesics of $\mathbb{R}P^2$ are periodic with the same period, the normalized (co)-geodesic flow induces a Hamiltonian $S^1$-action on the cotangent bundle. The boundary of the cotangent discs may be symplectically cut, or in other words, reduced, to a symplectic sphere. Thus, by using symplectic cut, we are able to replace a Lagrangian $\mathbb{R}P^2$ with a symplectic $(+4)$-sphere. In the case that the Lagrangian $\mathbb{R}P^2$ lies in $\mathbb{C}P^2$ this process transforms $\mathbb{C}P^2$ to $S^2\times S^2$. This is the content of 
\begin{proposition}
\label{cohodiffeo}
Let $(\widetilde{M}_1,\omega_1)$ and $(\widetilde{M}_2,\omega_2)$ be two symplectic manifolds that are obtained from surgery on Lagrangians $L_1,L_2$ in $\mathbb{C}P^2$, disjoint from a symplectic $(+4)$-sphere $S$. Then $(\widetilde{M}_1,\omega_1)$ is symplectomorphic to $(\widetilde{M}_2,\omega_2)$. In particular, both are symplectomorphic to $(S^2\times S^2, (1+\lambda)\sigma\oplus\sigma)$ with $\lambda>0$.
\end{proposition}
\begin{proof}
The manifolds $(\widetilde{M}_i,\omega_i)$ carry no $(-1)$-symplectic sphere and therefore, by a theorem of McDuff (see Theorem $9.4.1$ in \cite{McDS}), both are symplectomorphic to a symplectically ruled manifold. Since both contain the same $(+4)$-symplectic sphere (coming from $S$) and since we can perform the surgery on disc subbundles of the normal bundle of the $L_i$'s with the same radius $r$, we see that the $\omega_i$ represent the same cohomology class. Another theorem of McDuff (for example, Theorem $2.3$ in \cite{LaMcD}) states that any two cohomologous forms on a symplectically ruled surface are diffeomorphic. Thus, the $(\widetilde{M}_i,\omega_i)$ are symplectomorphic.\par
The last statement of the theorem follows by the classification of symplectic forms on $S^2\times S^2$ as done in \cite{Ab}. $\square$
\end{proof}


\subsection{Lagrangian $\mathbb{R}P^2$ and symplectic spheres in $\mathbb{C}P^2$}
We will now prove two \say{dual} results about $\mathbb{C}P^2$. The first claims that two symplectic spheres in $\mathbb{C}P^2$, disjoint from a Lagrangian $\mathbb{R}P^2$, may be symplectically isotoped while leaving the Lagrangian fixed. The second result makes the \say{opposite} claim, namely that two Lagrangians disjoint from a symplectic sphere can be symplectically isotoped to each other leaving the sphere fixed. 
\begin{proposition}\label{hindpropcp2}
Let $S_1,S_2$ be $(+4)$-symplectic spheres in $\mathbb{C}P^2$, disjoint from $L$, a Lagrangian $\mathbb{R}P^2$. Then, there exists a symplectomorphism $\psi$ of $\mathbb{C}P^2$ mapping $S_1$ to $S_2$ and fixing $L$ pointwise.
\end{proposition}
\begin{proof}
Since the symplectic spheres are disjoint from $L$, there exists a sufficiently small $r$ such that the symplectic tubular neighborhood of $L$ of radius $r$ is again disjoint from the $S_i$. Performing a symplectic cut with radius $r$ as described in the previous section, we end up with an $S^2\times S^2$, where $L$ is now an embedded symplectic sphere $\widetilde{S}$ (in $S^2\times S^2$). Using Proposition $\ref{hindtheorem}$ we construct a symplectic isotopy between $S_1$ and $S_2$ seen as submanifolds of $S^2\times S^2$ but, since the isotopy stays away from a neighborhood of $\widetilde{S}$, it can (and will) be seen as an isotopy $S_t$ between $S_1,S_2$ in $\mathbb{C}P^2$, staying away from $L$. We can extend this isotopy to a neighborhood of $S_t$ and then also trivially extend it to a neighborhood of $L$, which stays fixed as $t$ varies. Then using Banyaga's Extension Theorem, we can find symplectomorphisms $\phi_t$ that extend the isotopy $S_t$. Therefore $\phi_1$ is the desired map. $\square$
\end{proof}

\begin{proposition}\label{lagmap}
Let $L_1,L_2$ be two Lagrangian embeddings of $\mathbb{R}P^2$ in $\mathbb{C}P^2$ and let $S$ be a degree $2$ symplectic sphere, disjoint from the $L_i$. Then, there exists a symplectomorphism $\psi:\mathbb{C}P^2\rightarrow \mathbb{C}P^2$ such that $\psi(L_1)=L_2$ and $\psi=id$ in a neighborhood of $S$.
\end{proposition}
\begin{proof}
First, let us show that we can map $L_1$ to $L_2$. Consider each $L_i$ sitting in $\mathbb{C}P^2$. There exists a sufficiently small $r>0$ such that the radius $r$ tubular neighborhood of $L_i$, denoted by $\nu L_i$, is disjoint from $S$. By removing the $\nu L_i$ from $\mathbb{C}P^2$, and then reducing with the relevant $S^1$-action the boundary of both the tube and the remainder of $\mathbb{C}P^2$, for each $L_i$ we get two new symplectic manifolds, one coming from the reduced tube, which we denote by $\widetilde{N}_i$ and the other from the reduced $\mathbb{C}P^2$, which we denote by $\widetilde{M}_i$. As explained in the beginning of this section, both carry a symplectic sphere $\widetilde{S}_i$ coming from $L_i$, but with opposite oriented normal bundles. Now, we use Theorem $\ref{cohodiffeo}$ to find a symplectomorphism $\psi:\widetilde{M}_1\rightarrow \widetilde{M}_2$. Using Theorem $\ref{tracsy}$ we find a symplectomorphism $\phi$ of $\widetilde{M}_2$ such that $\phi(\psi(\widetilde{S}_1))=\widetilde{S}_2$. Thus, $\widetilde{\phi}=\phi\circ\psi$ is a symplectomorphism $\widetilde{M}_1\rightarrow \widetilde{M}_2$ mapping $\widetilde{S}_1$ to $\widetilde{S}_2$. Symplectically summing, again \textit{\'a la Gompf}, $(\widetilde{N}_i,\widetilde{S}_i)$ with $(\widetilde{M}_i,\widetilde{S}_i)$ we get a map $\rho:\mathbb{C}P^2\rightarrow \mathbb{C}P^2$ such that $\rho(L_1)=L_2$.\par
We now have to correct the map $\rho$ so it also fixes $S$. Since the $L_i$ are disjoint from $S$, $\rho(S)$ is also disjoint from $L_2$. Thus, we can apply Proposition $\ref{hindpropcp2}$ to those manifolds to get a new map $\xi$ that maps $\rho(S)$ to $S$ and preserves $L_2$. Therefore the map $\xi\circ\rho$ is -almost- the desired symplectomorphism, since $\xi(\rho(L_1))=\xi(L_2)=L_2$ and $\xi(\rho(S))=S$. \par 
Finally, since $\xi\circ\rho$ fixes $S$, a further isotopy can be made to fix a small neighborhood of it. To see this, notice that the symplectomorphism group of $\mathbb{C}P^2$ is connected and since $\mathbb{C}P^2$ is simply connected, we have that the map $\xi\circ\rho$ can be joined to the identity via Hamiltonian maps given by the functions $H_t$. We then localize $H_t$ around $S$ and thus the time $1$ map of the corresponding Hamiltonian flow is a symplectomorphism fixing pointwise a neighborhood of $S$.
\end{proof}
Combining the two results, we get the general
\begin{Theorem}$\label{sympair}$
Let $(L,S)$ be a disjoint pair consisting of a Lagrangian $\mathbb{R}P^2$ and a degree $2$ symplectic sphere, both inside $\mathbb{C}P^2$. Given any other such pair $(L',S')$, there exists a symplectomorphism $\psi$ mapping the first pair to the second, i.e. $\psi(L)=L'$ and $\psi(S)=S'$.
\end{Theorem}
\begin{proof}
By Proposition $\ref{lagmap}$, there exists a map $\psi'$ such that $\psi'(L)=L'$. Since $L$ and $S$ are disjoint $\psi'(S)$ and $S'$ are disjoint from $L'$ and therefore Proposition $\ref{hindpropcp2}$ implies that there exists a symplectomorphism $\phi$ fixing a neighborhood of $L'$ and joining $\psi'(S)$ and $S'$. Thus, the map $\psi=\phi\circ\psi'$ is the desired symplectomorphism between the pairs, since $\psi(S)=\phi(\psi'(S))=S'$ and $\psi(L)=\phi(L')=L'$. $\square$
\end{proof}

==> maintheorem.tex <==
Putting all the above together, the desired result becomes trivial.
\begin{Theorem}\label{maintheorem}
Let $L_1$ and $L_2$ be embedded Lagrangian submanifolds of $T^*\mathbb{R}P^2$ which are diffeomorphic to $\mathbb{R}P^2$. There exists a compactly supported Hamiltonian isotopy $H_t$ such that $H_1(L_1)=L_2$.
\end{Theorem}
\begin{proof}
Since the Lagrangians are compact, they live inside some cotangent disc bundle of radius $r$. We will compactify this disc bundle to $\mathbb{C}P^2$, where the boundary of the bundle is mapped to a degree $2$ symplectic sphere $S$ (Theorem $\ref{compacttheorem})$. Thus, we consider the Lagrangians $L_1$ and $L_2$ as living in the complement of $S$. Now, we can find a symplectomorphism $\psi$ of $\mathbb{C}P^2$ such that $\psi(L_1)=L_2$ and $\psi=id$ in a neighborhood of $S$ (Theorem $\ref{sympair}$). Therefore $\psi$ can be seen as a compactly supported symplectomorphism of $T^*\mathbb{R}P^2$ mapping $L_1$ to $L_2$.\par
The above symplectomorphism group has the homotopy type of the discrete group $\mathbb{Z}$, where $\pi_0$ is generated by a Dehn Twist $\bar\tau$ along the zero section $0_s$ (Corollary $\ref{dehntwist}$). In particular, $\bar\tau(0_s)=0_s$. Without loss of generality, we will assume that $L_2=0_s$. Thus, $\psi$ can be written as $\psi=\bar\tau\circ\eta_1$
where $\eta_t$ is a smooth path joining $\eta_1$ and the identity. Since $\bar\tau(0_s)=0_s$, we have that $\eta_1(L_1)=0_s$ therefore $\eta_t$ is the desired Hamiltonian isotopy mapping $L_1$ to $L_2$. $\square$
\end{proof}
